Analyzing Accuracy Loss in Randomized Smoothing Defenses

Recent advances in machine learning (ML) algorithms, especially deep neural networks (DNNs), have demonstrated remarkable success (sometimes exceeding human-level performance) on several tasks, including face and speech recognition. However, ML algorithms are vulnerable to \emph{adversarial attacks}, such test-time, training-time, and backdoor attacks. In test-time attacks an adversary crafts adversarial examples, which are specially crafted perturbations imperceptible to humans which, when added to an input example, force a machine learning model to misclassify the given input example. Adversarial examples are a concern when deploying ML algorithms in critical contexts, such as information security and autonomous driving. Researchers have responded with a plethora of defenses. One promising defense is \emph{randomized smoothing} in which a classifier's prediction is smoothed by adding random noise to the input example we wish to classify. In this paper, we theoretically and empirically explore randomized smoothing. We investigate the effect of randomized smoothing on the feasible hypotheses space, and show that for some noise levels the set of hypotheses which are feasible shrinks due to smoothing, giving one reason why the natural accuracy drops after smoothing. To perform our analysis, we introduce a model for randomized smoothing which abstracts away specifics, such as the exact distribution of the noise. We complement our theoretical results with extensive experiments.

==> src/50_technicalLemmas.tex <==
\section{Technical Definitions, Lemmas, and Theorems}

\begin{definition}\label{def:lossFunction}
Let $\hypothesisClass = \s{\model : \norm{\model}_2 \leq \modelNormBound}$ be our hypothesis class and let $\labeledInputSpace = \inputSpace \times \outputSpace$ be the examples domain.  Assume that the loss function $\ell : \hypothesisClass \times \inputSpace \to \realNumbers$ is of the form

\begin{equation}
    \loss(\model,(\sample,\sampleLabel)) = \placeholderFunc(\dotproduct{\model,\sample},\sampleLabel)
\end{equation}
where $\placeholderFunc : \realNumbers \times \outputSpace \to \realNumbers$ is such that for all $\sampleLabel \in \outputSpace$, the scalar function $\placeholder \mapsto \placeholderFunc(\placeholder,\sampleLabel)$ is $\lossLipschitzConstant$-Lipschitz.
\end{definition}


% \begin{theorem}[Theorem 26.12 from \cite{shalev2014understanding}]
% Suppose that $\sampleDist$ is a distribution over $\inputSpace \times \outputSpace$ such that with probability $1$, we have 
% $\norm{\sample}_2 \leq \inputNormBound$.  Let $\hypothesisClass = \s{\model : \norm{\model}_2 \leq \modelNormBound}$ and let $\loss : \hypothesisClass \times \labeledInputSpace \to \realNumbers$ be a loss function of the form given in \cref{def:lossFunction} such that for all $\sampleLabel \in \outputSpace$, the scalar function $\placeholder \mapsto \placeholderFunc(\placeholder,\sampleLabel)$ is $\lossLipschitzConstant$-Lipschitz and such that $\max_{\placeholder \in \br{-\modelNormBound\inputNormBound,\modelNormBound\inputNormBound}}\abs{\placeholderFunc(\placeholder,\sampleLabel)} \leq \lossBound$.  Then for any $\confidence \in \p{0,1}$, with probability of at least $1-\confidence$ over the choice of an i.i.d. sample of size $\numSamples$.

% \begin{equation}
%     \forall\model\in\hypothesisClass, \quad 
% \end{equation}
% \end{theorem}


% \begin{theorem}[Theorem 14 from \cite{xu2009robustness}]\label{thm:XuThm14}
% Suppose the kernel function has the form $\kernel(\vec{\placeholder},\vec{\placeholder}') = \placeholderFunc(\norm{\vec{\placeholder}-\vec{\placeholder}'})$ (where $\norm{\cdot}$ is an arbitrary norm) with $\placeholderFunc : \realNumbers^+ \to \realNumbers$ a decreasing function.  Denote by $\rkhsSpace$ the space of $\kernel(\cdot,\cdot)$ and $\featureMapping(\cdot)$ the corresponding feature mapping.  Then we have for any $\sample \in \realNumbers^\dimension$, $\model \in \rkhsSpace$ and $c > 0$,

% \begin{equation}
% \sup_{\norm{\perturbation}\leq c}\dotproduct{\model,\featureMapping(\sample-\perturbation)} = \sup_{\norm{\perturbation}_\rkhsSpace \leq \sqrt{2\placeholderFunc(0) - 2\placeholderFunc(c)}}\dotproduct{\model,\featureMapping(\sample )+ \perturbation_{\rkhsSpace}}
% \end{equation}

% where from $\vec{\placeholder} \in \rkhsSpace$
% \begin{equation}
%     \norm{\vec{\placeholder}_\rkhsSpace = \sqrt{\dotproduct{\vec{\placeholder},\vec{\placeholder}}}}
% \end{equation}
% \end{theorem}


% \begin{definition}[Growth Function (Section 3.2 of \cite{anthony2009neural})]
%   Consider a finite subset $\trainingData{}$ of input space $\inputSpace$.  For a function class $\hypothesisClass$, the restriction of $\hypothesisClass$ to the set $\trainingData{}$ is denoted by $\hypothesisClass_{\vert\trainingData{}}$.  If $\hypothesisClass_{\vert\trainingData{}}$ is the set of all functions from $\trainingData{}$ to $\s{0,1}$, then clearly $\hypothesisClass$ is as powerful as it can be in classifying the points in $\trainingData{}$.  We can view the cardinality of $\hypothesisClass_{\vert\trainingData{}}$ (and in particular, how it compares with $2^{\abs{\trainingData{}}}$) as a measure of the classification complexity of $\hypothesisClass$ with respect to the set $\trainingData{}$

%   The \emph{growth function} of $\hypothesisClass$, $\growthFunctionClass : \naturalNumbers \to \naturalNumbers$, is defined as
% \begin{equation}
%   \growthFunctionClass(\sampleComplexity{}) \coloneqq \max\s{\abs{\hypothesisClass_{\vert \trainingData{}}} : \trainingData{} \subset \inputSpace \text{ and } \abs{\trainingData{}} = \sampleComplexity{}}
% \end{equation}

% \end{definition}

% \begin{definition}[Vapnik-Chervonenkis Dimension (Section 3.3 of \cite{anthony2009neural})]
%  The Vapnik-Chervonenkis Dimension (VC-Dimension) is the largest value of $\sampleComplexity{}$ for which the growth function $\growthFunctionClass(\sampleComplexity{})$ equals $2^{\sampleComplexity{}}$
% \end{definition}

% \begin{definition}[Maximum Discrepancy (from \cite{bartlett2002rademacher})]
%   Let $\placeholderDist$ be a probability distribution on a set $\inputSpace$ and suppose that $\sample_1,\sample_2,\hdots,\sample_{\numSamples}$ are independent samples selected according to $\placeholderDist$.  Let $\hypothesisClass$ be a class of functions mapping from $\inputSpace$ to $\realNumbers$.  Define the \emph{maximum discrepancy} of $\hypothesisClass$ as the random variable:
%   \begin{equation}
%     \discrepancyHat_{\numSamples}(\hypothesisClass) \coloneqq \sup_{\hyp \in \hypothesisClass}\p*{\frac{2}{\numSamples}\sum_{i=1}^{\numSamples/2}\hyp\p{\sample_i} - \frac{2}{\numSamples}\sum_{i=\numSamples/2 + 1}^{\numSamples}\hyp\p{\sample_i}}
%   \end{equation}

%   Denote the expected maximum discrepancy of $\hypothesisClass$ by $\discrepancy_{\numSamples}\p{\hypothesisClass} \coloneqq \E{\discrepancyHat_{\numSamples}\p{\hypothesisClass}}$
% \end{definition}

\begin{definition}[Rademacher Complexity (from \cite{bartlett2002rademacher})]
    Let $\placeholderDist$ be a probability distribution on a set $\inputSpace$ and suppose that $\trainingData{} = \s{\sample_1,\sample_2,\hdots,\sample_{\numSamples}}$ is a set of $\numSamples$ independent samples selected according to $\placeholderDist$.  Let $\hypothesisClass$ be a class of functions mapping from $\inputSpace$ to $\realNumbers$.  Define the random variable:
    \begin{equation}
      \rademacherComplexityHat_{\numSamples}\p*{\hypothesisClass \circ \trainingData{}} \definedAs \E{\sup_{\hyp \in \hypothesisClass}\frac{2}{\numSamples}\sum_{i=1}^{\numSamples}\rademacherVariable_i\hyp\p{\sample_i}}
    \end{equation}
    where $\rademacherVariable_1,\hdots,\rademacherVariable_\numSamples$ are independent uniform $\s{\pm 1}$-valued random variables.

    The \emph{Rademacher Complexity} of $\hypothesisClass$ is $\rademacherComplexity_{\numSamples}(\hypothesisClass \circ \trainingData{}) \coloneqq \E{  \rademacherComplexityHat_{\numSamples}\p*{\hypothesisClass \circ \trainingData{}}}$
\end{definition}

% \begin{definition}[Gaussian Complexity]
%   Let $\placeholderDist$ be a probability distribution on a set $\inputSpace$ and suppose that $\trainingData{} = \s{\sample_1,\sample_2,\hdots,\sample_{\numSamples}}$ is a set of $\numSamples$ independent samples selected according to $\placeholderDist$.  Let $\hypothesisClass$ be a class of functions mapping from $\inputSpace$ to $\realNumbers$.  Define the random variable:
%   \begin{equation}
%     \gaussianComplexityHat_{\numSamples}\p*{\hypothesisClass \circ \trainingData{}} \coloneqq \E{\sup_{\hyp \in \hypothesisClass}\frac{2}{\numSamples}\sum_{i=1}^{\numSamples}\gaussianVariable_i\hyp\p{\sample_i}}
%   \end{equation}
%   where $\gaussianVariable_1,\hdots,\gaussianVariable_\numSamples$ are independent Gaussian $\gaussianDist(0,1)$ random variables.

%   The \emph{Gaussian Complexity} of $\hypothesisClass$ is $\gaussianComplexity_{\numSamples}(\hypothesisClass \circ \trainingData{}) \coloneqq \E{  \gaussianComplexityHat_{\numSamples}\p*{\hypothesisClass \circ \trainingData{}}}$
% \end{definition}
\begin{definition}[Log-Concave Distribution]

    We source our definition of Log-Concave Distributions from Saumard and Wellner~\cite{saumard2014log}.

    A density function $\placeholderDist$ with respect to Lebesgue measure $\lebesgueMeasure$ on $(\realNumbers^\dimension,\algebra^\dimension)$ is log-concave if $\placeholderDist=e^{-\placeholderFunc}$ where $\placeholderFunc$ is a convex function from $\realNumbers^\dimension$ to $(-\infty,\infty]$
\end{definition}

% \begin{definition}
%     For any $\standardDeviation^2 > 0$, define the class of strongly log-concave densities with variance parameter $\standardDeviation^2$, or $\slc_1(\standardDeviation^2,\dimension)$ to be the collection of density functions $\placeholderDist$ of the form 
%     \begin{equation}
%         \placeholderDist(\sample) = \placeholderFunc(\sample)\normalDistribution_{\zerosDimension,\standardDeviation^2\identityMatrix}(\sample)
%     \end{equation}
    
%     If a random vector $\vec{\placeholder}$ has a density $\placeholderDist$ of this form, then we also say that $\vec{\placeholder}$ is strongly log-concave
% \end{definition}

% \begin{definition}
%     Let $\covarianceMatrix$ be a $\dimension \times \dimension$ positive definite matrix and let $\vec{\placeholder}'\in \realNumbers^\dimension$.  We say that a random vector $\vec{\placeholder}$ and its density function $\placeholderDist$ are strongly log-concave and write $\placeholderDist \in \slc_2(\vec{\placeholder}',\covarianceMatrix,\dimension)$ if
%     \begin{equation}
%         \placeholderDist(\vec{\placeholder})= \placeholderFunc(\vec{\placeholder})\normalDistribution_{\vec{\placeholder}',\standardDeviation^2\identityMatrix}(\vec{\placeholder})
%     \end{equation}
% \end{definition}

% \subsection{Schaefer's Dichotomy Theorem}

% \subsubsection{Theorem Statement}
% \begin{theorem}[Schaefer's Dichotomy Theorem \cite{schaefer1978complexity}]
% Let $\logicalRelationSet = \s{\logicalRelation_1,\hdots,\logicalRelation_{\logicalRelationNumber}}$ be a finite set of logical relations.  If $\logicalRelationSet$ satisfies one of the conditions below, then $\SAT(\logicalRelationSet)$ is polynomial-time decidable.  Otherwise, $\SAT(\logicalRelationSet)$ is \NP-complete:
% \begin{enumerate}[label=\upshape(\roman*)]
%     \item Every relation in $\logicalRelationSet$ is $0$-valid.
%     \item Every relation in $\logicalRelationSet$ is $1$-valid.
%     \item Every relation in $\logicalRelationSet$ is weakly positive.
%     \item Every relation in $\logicalRelationSet$ is weakly-negative.
%     \item Every relation in $\logicalRelationSet$ is affine.
%     \item Every relation in $\logicalRelationSet$ is bijunctive.
%     \end{enumerate}
% \end{theorem}


% \subsubsection{Definitions related to Schaefer's Dichotomy Theorem}

% \begin{zvalidity}
% The logical relation $\logicalRelation$ is $0$-valid if $\p{0,\hdots,0}\in \logicalRelation$.
% \end{zvalidity}

% \begin{ovalidity}
% The logical relation $\logicalRelation$ is $1$-valid if $\p{1,\hdots,1}\in \logicalRelation$.
% \end{ovalidity}

% \begin{weaklyPositive}
% The logical relation $\logicalRelation$ is weakly positive if $\logicalRelation$ is logically equivalent to some Conjunctive Normal Form (CNF) formula having at most one negated variable in each conjunct.
% \end{weaklyPositive}
% \begin{weaklyNegative}
% The logical relation $\logicalRelation$ is weakly negative if $\logicalRelation$ is logically equivalent to some CNF formula having at most one unnegated variable in each conjunct.
% \end{weaklyNegative}
% \begin{bijunctive}
% A logical relation $\logicalRelation$ is bijunctive if $\logicalRelation$ is logically equivalent to some CNF formula having at most two literals in any conjunct.
% \end{bijunctive}
% \begin{affine}
% A logical relation $\logicalRelation$ is affine if $\logicalRelation$ is logically equivalent to some system of linear equations over the two-element field $\s{0,1}$; that is, if $\logicalRelation$ is logically equivalent to a conjunction of formulas of the form $\s{0=\placeholder_1\xor\placeholder_2\xor\hdots}$ and $\s{1=\placeholder_1\xor\placeholder_2\xor\hdots}$ where $\xor$ denotes addition modulo $2$.
% \end{affine}
% % \newtheorem*{zvalidity}{0-Valid}
% % \newtheorem*{ovlaidity}{1-valid}
% % \newtheorem*{weaklyPositive}{Weakly Positive}
% % \newtheorem*{weaklyNegative}{Weakly Negative}
% % \newtheorem*{bijunctive}{Bijunctive}
% % \newtheorem*{affine}{Affine}

==> src/81_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> src/algorithms/predict.tex <==
\begin{algorithm}
\caption{Prediction Function}\label{alg:cohenPredict}
\begin{algorithmic}[1]
\Procedure{Predict}{$\hyp, \sample, \noiseDist,\numDraws$}
\State $\predictions \gets \s{p_1,\hdots,p_{\numDraws}}$ \Comment{$\predictions$ is an index family}
\For{$\idx \in \s{1,\hdots,\numDraws}$}
\State $\predictions[\idx] \gets \hyp(\sample + \noiseInstance_i)$ \Comment{$\noiseInstance_i \overset{\text{i.i.d}}{\drawnFrom}\noiseDist$}
\EndFor\label{euclidendwhile}
\State $\prediction \gets \arg\max_{\placeholder \in \predictions} \sum_{\idx=1}^\numDraws \indicatorFunction\br{\predictions[\idx] = \placeholder}$
\State \textbf{return} $\prediction$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> src/pgfFigures/1drealizable.tex <==
\begin{tikzpicture}

\begin{axis}[no markers, domain=0:10, samples=100,
axis lines*=left, xlabel= $x_1$, ylabel= $x_2$,
height=6cm, width=10cm,
enlargelimits=false, clip=false, axis on top,
grid = major]
\begin{scope}[blend group=soft light]
\addplot [fill=cyan!20, draw=black, domain=-3:3] {gauss(0,1)} \closedcycle;
\addplot [fill=orange!10, draw=black, domain=-3:3] {-gauss(1,1)} \closedcycle;
\addplot [fill=green!10 , draw=black, domain=-3:3] {-gauss(-1,1)} \closedcycle;
\end{scope}
\end{axis}
\end{tikzpicture}

==> src/pgfFigures/NoSmoothing.tex <==
\begin{tikzpicture}
	\begin{axis}[%
	scatter/classes={%
		a={mark=*,blue},%
		b={mark=triangle*,green},%
		c={mark=o,draw=black}},
		d={mark=triangle*,orange},%
		e={mark=triangle*,pink},%
		f={mark=triangle*,teal},%
		g={mark=triangle*,yellow},%
		a={mark=square*,blue},%
		b={mark=triangle*,green},%
		d={mark=triangle*,orange},%
		e={mark=triangle*,pink},%
		f={mark=triangle*,teal},%
		g={mark=triangle*,yellow},%
		a={mark=square*,blue},%
		b={mark=triangle*,green},%
		d={mark=triangle*,orange},%
		e={mark=triangle*,pink},%
		f={mark=triangle*,teal},%
		g={mark=triangle*,yellow}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.1   0.15   a 
0.45  0.27   b 
0.02  0.17   c 
0.06  0.1    d 
0.9   0.5    e 
0.5   0.3    f 
0.85  0.52   g 
0.12  0.05   h 
0.73  0.45   i 
0.53  0.25   j 
0.76  0.5    k 
0.55  0.32   l
	};
	\end{axis}
\end{tikzpicture}
